Adversarial Example Does Good: Preventing Painting Imitation from Diffusion Models via Adversarial Examples

Recently, Diffusion Models (DMs) boost a wave in AI for Art yet raise new copyright concerns, where infringers benefit from using unauthorized paintings to train DMs to generate novel paintings in a similar style. To address these emerging copyright violations, in this paper, we are the first to explore and propose to utilize adversarial examples for DMs to protect human-created artworks. Specifically, we first build a theoretical framework to define and evaluate the adversarial examples for DMs. Then, based on this framework, we design a novel algorithm, named AdvDM, which exploits a Monte-Carlo estimation of adversarial examples for DMs by optimizing upon different latent variables sampled from the reverse process of DMs. Extensive experiments show that the generated adversarial examples can effectively hinder DMs from extracting their features. Therefore, our method can be a powerful tool for human artists to protect their copyright against infringers equipped with DM-based AI-for-Art applications. The code of our method is available on GitHub: https://github.com/mist-project/mist.git.

==> inputs/nonsense.tex <==
\section{Nonsense}
\subsection{Understanding Adversarial Examples for Generative Models}
\label{sec:understanding}
A straightforward explanation of Definition~\ref{def:1} is the image $x'$ with a high probability to be recognized as real data and a low probability to be sampled from the generative model. Let $q(x)$ and $p_\theta (x)$ be the distributions of real data and generated data respectively. Note that the value of $q(x)$ indicates the probability that $x$ is a real image and that of $p_{\theta}(x)$ indicates the probability that $x$ is sampled by the generative model. Following the explanation, an adversarial example $x'$ can be then characterized by a high value of $q(x')$ and a low value of $p_{\theta}(x')$ and can be regarded as out-of-distribution data for generative model $\theta$~\cite{nalisnick2018deep}. To better illustrate the explanation, we start from an implicit assumption on out-of-distribution in the modeling of adversarial learning.
\begin{assumption}[\textbf{Smoothness of $q(x)$}]
\label{amp:1}
Given a real image $x$ and a perturbation $\delta$ with $\delta\leq\epsilon$, we have $q(x+\delta)\approx q(x)$. Here, $\epsilon$ is a tiny constant often smaller than $\frac{10}{255}$ in practice.   
% \textcolor{red}{Given a real image $x$, for $\forall \epsilon > 0$, there exists a perturbation bound $\epsilon > 0$, for $\forall \delta$ with $ - \epsilon < \delta < \epsilon$, we have $|q(x + \delta) - q(x)| < \epsilon$.}
\end{assumption}
% \textcolor{red}{In practice, the constant $\epsilon$ is often smaller than $\frac{1}{255}$.}
The assumption is held on the foundation that a tiny perturbation would not change the image semantics and the probability to be recognized as a real image by humans~\cite{}. Based on the assumption, $q(x)$ is approximately constant on a small neighborhood of the real image $x$. 

Although the generative model $\theta$ is optimized to approximate $q(x)$ by $p_{\theta}(x)$, the smoothness of $p_{\theta}(x)$ is not guaranteed as that of $q(x)$ demonstrated in Assumption~\ref{amp:1}, for $p_{\theta}(x)$ is optimized to behaves similar to $q(x)$ only on the data point $x$. On the contrary, neural networks used in the construction of $p_{\theta}(x)$ are believed to be highly unsmooth~\cite{} and thus impossible to be steady in the neighborhood of the real image $x$. Although $\frac{p_{\theta}(x)}{q(x)}\approx 1$ after optimizing $\theta$, we may have $\frac{p_{\theta}(x+\delta)}{q(x+\delta)}\ll 1$ by carefully picking a tiny perturbation $\delta$, which maintains $q(x+\delta)\approx q(x)$. This is exactly formulated by Definition~\ref{def:1}.

\begin{figure}[th]
\vskip 0.2in
\begin{center}
\includegraphics[width=0.99\columnwidth]{figs/demo.pdf}
\caption{Finding adversarial example $x'$ for real image $x$}
\label{fig:demo}
\end{center}
\vskip -0.2in
\end{figure}

Figure~\ref{fig:demo} demonstrates the basic pattern of finding adversarial examples. $q(x)$ stays approximately constant in a small neighborhood with a radius of $\epsilon$, while $p_{\theta}(x)$ drops dramatically along some direction. This difference makes it possible to find an $x'$ in the $\epsilon$-neighborhood of $x$ with high $q(x')$ and low $p_{\theta}(x')$.

==> inputs/visualization_of_ablation_study.tex <==
\section{visualization of experiments in ablation study}
We also provide the visualization of the generated images based on adversarial examples generated under different budgets . From Figure \ref{vis_epi}, we can observe the semantic information of the airplane becomes more and more unclear.

\begin{figure}[ht]

\begin{center}
\includegraphics[width=0.48\textwidth]{figs/vis_epi_tight.png}
\caption{Visualization of generated images under AdvDM under different budgets. First column: The adversarial examples. The second to the sixth column: The image generated using the pseudo-word derived from the adversarial examples.}
\label{vis_epi}

\end{center}

\end{figure}

==> inputs/visualization_of_style_transferring.tex <==
\section{More Qualitative Results on Style Transferring}
\label{sty2}
We  provide more examples of how AdvDM can disturb style transferring in Figure \ref{style2}.

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\includegraphics[width=0.49\textwidth]{figs/more_visualization/merge_source_tight.pdf}
\caption{One group of the clean examples and adversarial examples in Lsun-cat, Lsun-sheep, Lsun-airplane  dataset. The top row shows the clean examples while the bottom row shows the adversarial examples under AdvDM.}
\label{merge_source}
\end{center}
\vskip -0.2in
\end{figure}

\begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\includegraphics[width=0.99\textwidth]{figs/style_transfer_v3_part2.png}
\caption{AdvDM under style transfer in Wiki-art datasets. In each group, the middle images in the top row refer to the generated images under clean training samples while the middle images in the bottom row indicate the generated images under attacked training samples.}
\label{style2}
\end{center}
\vskip -0.2in
\end{figure*}


==> inputs/visualization_of_textual_inversion.tex <==
\section{Visualization on text-to-image generation based on textual inversion}
\label{vis-txt2img}
We  provide  visualization of how AdvDM can disturb text-to-image generation in different datasets. The setting is the same as the one mentioned in Section \ref{sam}.
One group of the given images for deriving the pseudo-words for each dataset is shown in Figure \ref{merge_source}. The generation result based on clean images and adversarial images in shown in Figure \ref{mergegen}.
\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\includegraphics[width=0.49\textwidth]{figs/more_visualization/merge_source_extend.pdf}
\caption{One group of the clean images and adversairal images in Lsun-cat, Lsun-sheep, Lsun-airplane  dataset. The top row shows the clean examples while the bottom row shows the adversarial examples under AdvDM.}
\label{merge_source}
\end{center}
\vskip -0.2in
\end{figure}
% \begin{figure}
% \vskip 0.2in
% \begin{center}
% \includegraphics[width=0.49\textwidth]{figs/more_visualization/merge_source.pdf}
% \caption{One group of the clean images and adversairal images in Lsun-cat, Lsun-sheep , Lsun-airplane  dataset. The top row shows the clean examples while the bottom row shows the adversarial examples under AdvDM.}
% \label{merge_source}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \subsection{Lsun-cat}

% One group of the given images for deriving the pseudo-words for Lsun-cat dataset is shown in Figure \ref{catsource}. The generation result based on clean images and adversarial images in shown in Figure \ref{catgener}.

% \begin{figure}[htbp]
% \vskip 0.2in
% \begin{center}
% \includegraphics[width=0.48\textwidth]{figs/more_visualization/cat_source.png}
% \caption{One group of the images in Lsun-cat dataset. The top row shows the clean examples while the bottom row shows the adversarial examples under AdvDM.}
% \label{catsource}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \begin{figure*}[htbp]
%  \begin{center}
%     \centering
%     \subfigure[Generation based on clean examples]{
%         \includegraphics[width=0.48\linewidth]{figs/more_visualization/6_cats_clean.jpg}}
%     \subfigure[Generation based on adversarial examples]{
%         \includegraphics[width=0.48\linewidth]{figs/more_visualization/6_cats.jpg}}

%     \caption{(a) Text-to-image generation based on textual inversion for clean examples. (b) Text-to-image generation based on textual inversion for clean examples.  The step-wise perturbation budget $\alpha$ is fixed to 1/255 and the overall perturbation budget $\epsilon$ is fixed to 8/255.}

%     \label{catgener}
% \vskip -0.2in
% \end{center}
% \vskip -0.2in
% \end{figure*}
% \subsection{Lsun-sheep}


% One group of the given images for deriving the pseudo-words for Lsun-sheep dataset is shown in Figure \ref{sheepsource}. The generation result based on clean images and adversarial images in shown in Figure \ref{sheepgener}.

% \begin{figure}[htbp]
% \vskip 0.2in
% \begin{center}
% \includegraphics[width=0.48\textwidth]{figs/more_visualization/sheep_source.png}
% \caption{One group of the images in Lsun-sheep dataset. The top row shows the clean examples while the bottom row shows the adversarial examples under AdvDM.}
% \label{sheepsource}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \begin{figure*}[htbp]
% %  \begin{center}
%     \centering
%     \subfigure[Generation based on clean examples]{
%         \includegraphics[width=0.48\linewidth]{figs/more_visualization/3_sheep_clean.jpg}}
%     \subfigure[Generation based on adversarial examples]{
%         \includegraphics[width=0.48\linewidth]{figs/more_visualization/3_sheep.jpg}}

%     \caption{(a) Text-to-image generation based on textual inversion for clean examples. (b) Text-to-image generation based on textual inversion for clean examples.  The step-wise perturbation budget $\alpha$ is fixed to 1/255 and the overall perturbation budget $\epsilon$ is fixed to 8/255.}

%     \label{sheepgener}
% \vskip -0.2in
% \end{center}
% \vskip -0.2in
% \end{figure*}

% \subsection{Lsun-airplane}


% One group of the given images for deriving the pseudo-words for Lsun-airplane dataset is shown in Figure \ref{airplanesource}. The generation result based on clean images and adversarial images in shown in Figure \ref{airplanegener}.

% \begin{figure}[htbp]
% \vskip 0.2in
% \begin{center}
% \includegraphics[width=0.48\textwidth]{figs/more_visualization/airplane_source.png}
% \caption{One group of the images in Lsun-airplane dataset. The top row shows the clean examples while the bottom row shows the adversarial examples under AdvDM.}
% \label{airplanesource}
% \end{center}
% \vskip -0.2in
% \end{figure}


\begin{figure*}[htbp]
\vskip 0.2in
\begin{center}
%\includegraphics[width=0.98\textwidth]{figs/more_visualization/summary_output.pdf}
\includegraphics[width=\textwidth]{figs/more_visualization/summary_output_extend.pdf}
\caption{Left: Text-to-image generation based on textual inversion for clean examples. Right: Text-to-image generation based on textual inversion for adversarial examples. }
\label{mergegen}
\end{center}
\vskip -0.2in
\end{figure*}

% \begin{figure*}[htbp]
%  \begin{center}
%     \centering
%     \subfigure[Generation based on clean examples]{
%         \includegraphics[width=0.48\linewidth]{figs/more_visualization/8_airplane_clean.jpg}}
%     \subfigure[Generation based on adversarial examples]{
%         \includegraphics[width=0.48\linewidth]{figs/more_visualization/8_airplane.jpg}}

%     \caption{(a) Text-to-image generation based on textual inversion for clean examples. (b) Text-to-image generation based on textual inversion for clean examples.  The step-wise perturbation budget $\alpha$ is fixed to 1/255 and the overall perturbation budget $\epsilon$ is fixed to 8/255.}

%     \label{airplanegener}
% \vskip -0.2in
% \end{center}
% \vskip -0.2in
% \end{figure*}
